DataRaceBench V1.4.1 and DataRaceBench-ML V0.1: Benchmark Suites for Data Race Detection

Data races pose a significant threat in multi-threaded parallel applications due to their negative impact on program correctness. DataRaceBench, an open-source benchmark suite, is specifically crafted to assess these data race detection tools in a systematic and measurable manner. Machine learning techniques have recently demonstrated considerable potential in high-performance computing (HPC) program analysis and optimization. However, these techniques require specialized data formats for training and refinement. This paper presents the latest update to DataRaceBench, incorporating new data race contributions from Wu et al. \cite{wu2023model}, and introduces a derived dataset named DataRaceBench-ML (DRB-ML) \cite{drbml}. DRB-ML aligns with the emerging trend of machine learning and large language models. Originating from DataRaceBench, this dataset includes detailed labels that denote the presence of a data race and provides comprehensive details of associated variables, such as variable names, line numbers, and the operation (read/write). Unique to DRB-ML, we have also integrated a series of tailored prompt-response pairs specifically designed for LLM fine-tuning.

==> sections/2-background.tex <==
% This section provides background information on key concepts such as machine learning, large language models, and DataRaceBench, setting the stage for the discussions to follow.
\subsection{Machine Learning and Large Language Models}
Machine learning harnesses algorithms and statistical models to carry out tasks. The performance of these models largely depends on the quality and quantity of the training data.
In particular, supervised learning models necessitate well-labeled and meticulously processed data for training. These models learn to establish mappings from inputs (features) to outputs (labels), optimizing internal parameters to reduce the deviation between the predicted and actual labels.

Large Language Models (LLMs) have emerged as a potent subclass within the broad spectrum of machine learning models. LLMs have achieved significant successes across diverse domains owing to their capacity to understand and generate text that is similar to human language. Their substantial size, typically determined by the number of parameters, enables them to grasp complex patterns and relationships within the data. However, to fine-tune these models for specific tasks, a dedicated dataset composed of prompt-response pairs is required. These pairs guide the initial learning process and provide corrective feedback, aiding in the enhancement of the model's comprehension and predictive accuracy.




\subsection{DataRaceBench}
DataRaceBench is an open-source benchmark suite developed to encapsulate a wide range of potential data race patterns in OpenMP programs. It serves as a comprehensive suite for evaluating the accuracy and overhead of various data race detection tools. Since its inception in 2017, DataRaceBench has become an essential resource for understanding and assessing the performance of different data race detection tools. DataRaceBench is publicly accessible on its \href{https://github.com/LLNL/dataracebench}{GitHub repo}. The latest version of DRB before this paper is DataRaceBench V1.4.0, which includes 181 microbenchmarks in C/C++.


Although DataRaceBench has proven to be a vital tool for assessing traditional data race detection methods, it exhibits certain limitations when employed for machine learning-based approaches. We address these limitations with our newly developed DataRaceBench-ML, which we discuss in the following sections.









% \begin{table}[h]
% \caption{Property labels of microbenchmarks in DRB}
% \label{tab:drb-features}
% \begin{tabular}{|l|l|}
% \hline
% Property labels for race-yes set & Property labels for race-no set      \\ \hline
% Y1: \small Unresolvable dependencies    & N1: \small Embarrassingly parallel          \\ \hline
% Y2: \small Missing data sharing clauses & N2: \small Use of data sharing clauses      \\ \hline
% Y3: \small Missing synchronization      & N3: \small Use of synchronization           \\ \hline
% Y4: \small SIMD data races              & N4: \small Use of SIMD directives           \\ \hline
% Y5: \small Accelerator data races       & N5: \small Use of accelerator directives    \\ \hline
% Y6: \small Undefined behaviors          & N6: \small Use of special language features \\ \hline
% Y7: \small Numerical kernel data races  & N7: \small Numerical kernels                \\ \hline
% \end{tabular}
% \end{table}












==> sections/3-approach.tex <==
In this section, we provide an in-depth overview of the DRB-ML dataset. 
\subsection{Enriching DataRaceBench with External Datasets}
\subsection{Formulating Feature Labels for the DRB-ML Dataset}
\subsection{Crafting Prompt-Response Pairs for LLM Fine-tuning}








\begin{lstlisting}[language=Python, caption=Basic prompt]
"
You are an HPC export. Detect the data race in the below code. You first answer "yes" or "no" for data race existence and follow with data race variable information.
{code to test}
"
\end{lstlisting}

\begin{lstlisting}[language=Python, caption= Prompt to check data dependence before checking data race]
"
You are an HPC export. Detect the data dependence in the below code first, then detect the data race. You first answer "yes" or "no" for data race existence and follow with data race variable information.
{code to test}
"
\end{lstlisting}

\begin{lstlisting}[language=Python, caption= Prompts to check data dependence before checking data race]
"You are an HPC export. Detect the data dependence in the below code.
{code to test}"
"Detect the data race in the above code. You first answer "yes" or "no" for data race existence and follow with data race variable information.
    "
\end{lstlisting}







==> sections/4-results.tex <==
In this section, we put the DataRaceBench-ML (DRB-ML) to the test with various LLMs.

\subsection{Experiment Setup}
To underscore the utility of DRB-ML, we devised two experiments deploying various widely-used LLMs. Our first experiment, Task 1, aimed at detecting data races with the help of LLMs. Task 2, on the other hand, focused on fine-tuning the LLMs specifically for data race detection. The following models were chosen for these tasks: GPT-3.5-turbo, GPT-4, and Llama2-7b.

% \begin{itemize}
%     \item GPT-3.5-turbo: An advanced iteration of the GPT-3 model by OpenAI, GPT-3.5-turbo showcases significant strides in language understanding and generation. With an astounding 175 billion parameters, it is adept at producing human-like text with a remarkable degree of coherence and complexity.
%     \item GPT-4: The successor to GPT-3.5, GPT-4 has pushed the boundaries of AI and Natural Language Processing (NLP) to a new level. It possesses a vastly augmented parameter count, culminating in an exceptional performance in terms of language understanding, contextual awareness, and generation. Its heightened capacity to decipher patterns in code presented as text makes it a compelling candidate for our data race detection experiments.
%     \item Llama 2: A cutting-edge open-source language model, Llama 2 serves as a comprehensive platform that enables users and developers to experiment and develop tools leveraging its foundational structure.
% \end{itemize}

Our experiments were conducted on a Dell workstation equipped with a dual Intel Xeon 6238 CPU operating at 2.10GHz, 128 GB main memory, 1TB SSD drive, and an NVIDIA Quadro RTX 6000 GPU with 24GB memory. To ensure consistent output across all models, we fixed the 'temperature' parameter for the LLMs at zero. Additionally, we limited the 'max\_token' value for outputs to 256, reserving a more significant token quota for inputs. For our evaluation, we emphasized metrics such as accuracy and F1-Score to gauge the effectiveness of each model in data race detection. Having outlined our experimental setup, we now delve into the results, elucidating the performance of each model under the tasks outlined.

\subsection{Data Race Detection with LLMs}
For the data race detection using LLMs, we designed an automated procedure, encapsulated in a script. This script systematically performs the following actions:
\begin{enumerate}
    \item Load the DRB-ML dataset.
    \item Apply a threshold to the "code\_len" label, filtering data with more 4000 tokens to ensure it aligns with the model's input size restrictions.
    \item Extract the "trimmed\_code" from the dataset. Using the template shown in Listing \ref{lst:prompt_example}, it crafts the prompt inputs for the LLMs.
    \item Compare the LLMs' output against the "data\_race" values present in DRB-ML to determine detection accuracy.
\end{enumerate}


% extract the "trimmed\_code" from DRB-ML and construct prompts. These prompts were then processed by the LLMs to detect any data races within the given code. Listing \ref{lst:dr_detection} provides an example of this process. We compared the output of the LLMs with the "data\_race" values from DRM-ML. The results of this comparison are detailed in Table \ref{tab:t1}.






\begin{lstlisting}[language=python, caption=prompt for LLMs to detect data race, label=lst:prompt_example]
{
"prompt": "You are an HPC export. Check if the given code contains a data race. If there is a data race, report the variable pairs causing the data race and the line number. {trimmed\_code}",
}
\end{lstlisting}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{LLMs comparison for data race detection. }
\label{tab:llm-res}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Model         & TP           & FP          & TN          & FN         & Recall         & Precision      & F1             \\ \hline
GPT-3.5 & 66           & 55          & 43          & 34         & 0.660          & 0.545          & 0.597          \\ \hline
GPT-4         & 77           & \textbf{28} & \textbf{70} & 23         & 0.770          & \textbf{0.733} & \textbf{0.751} \\ \hline
Llama2   & \textbf{100} & 98          & 0           & \textbf{0} & \textbf{1.000} & 0.505          & 0.671          \\ \hline
\end{tabular}
\end{table}

Table \ref{tab:llm-res} presents the results of data race detection using various LLMs. Out of the DRB-ML dataset, 198 data entries met the code length threshold criteria and were thus included in the inference tests. The labels provided by the DRB-ML dataset proved instrumental in underpinning the experiments. Notably, the GPT-4 model demonstrated superior performance in data race detection when compared to the other two LLMs. It's important to highlight that, for this particular test, we relied solely on the data race label for inference. However, the abundance and richness of labels in DRB-ML lay the groundwork for a plethora of machine learning-driven data race analysis tasks in the future.

\subsection{LLM Fine-tuning with DRB-ML}
A crucial aspect of the DataRaceBench-ML (DRB-ML) lies in its prompt-response pairs. These pairs are specifically crafted to serve as a training ground for Large Language Models (LLMs), guiding them in recognizing and interpreting data races within codes.

In orchestrating our fine-tuning experiments, we adopted a classic 80-20 split approach to the DRB-ML dataset. Specifically, 80\% of the DRB-ML codes and their corresponding prompt-response pairs were earmarked for the fine-tuning phase. The remaining 20\% was reserved for testing purposes, providing an evaluation ground to assess the true prowess of our tuned models on unfamiliar instances.


Using the prompt-response pairs from DRB-ML, we embarked on the task of fine-tuning the LLMs. This involved:
\begin{enumerate}
\item Loading the prompts and their corresponding responses from the DRB-ML dataset.
\item Integrating these pairs into the LLM's training regimen. A commonly used supervised fine-tuning process was used.
\item Evaluating the model's performance on new, unseen prompts to gauge its understanding and accuracy in detecting data races.
\end{enumerate}

Table \ref{tab:fine-tune} offers a comparative performance analysis.  After being fine-tuned with our dataset, the Llama2-7b model exhibited a remarkable improvement in its capabilities.


\begin{table}[]
\caption{Llama2-7b-chat fine-tuning with DRB-ML for data race detection}
\label{tab:fine-tune}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Model      & TP & FP & TN & FN & Recall & Precision & F1    \\ \hline
original   & 20 & 20 & 0  & 0  & 1.000  & 0.500     & 0.667 \\ \hline
fine-tuned & 20 & 15 & 3  & 2  & 0.909  & 0.571     & 0.702 \\ \hline
\end{tabular}
\end{table}
